Simulated Detector Performance at the Muon Collider

In this paper we report on the current status of studies on the expected performance for a detector designed to operate in a muon collider environment. Beam-induced backgrounds (BIB) represent the main challenge in the design of the detector and the event reconstruction algorithms. The current detector design aims to show that satisfactory performance can be achieved, while further optimizations are expected to significantly improve the overall performance. We present the characterization of the expected beam-induced background, describe the detector design and software used for detailed event simulations taking into account BIB effects. The expected performance of charged-particle reconstruction, jets, electrons, photons and muons is discussed, including an initial study on heavy-flavor jet tagging. A simple method to measure the delivered luminosity is also described. Overall, the proposed design and reconstruction algorithms can successfully reconstruct the high transverse-momentum objects needed to carry out a broad physics program.

==> other.tex <==
\note{Decide if to Talk/speculate about the ones we don't have results, e.g.: taus, non-prompt particles. Can alo mention  special reconstruction / requirements / considerations for things as short tracks and timing considerations for heavy/slow particles}.

%Taus

%non-prompt particles

%short tracks

%slow particles considerations (timing, dE/dx)


==> physics.tex <==
Available selected physics results based on full simulation.
If planning standalone publication, one can add a short paragraph-long subsection with summary and reference the standalone publication.
If not planning a separate publication, one can add a dedicated subsection with the details.

Current table of contents represent just a possible list (addition / subtractions possible).

\subsection{$H\to ZZ\to 4l$}
\hfill\textit{Angela Zaza, Chiara Aim\'e, Rosamaria Venditti, Filippo Errico}\\
\\In this section, a feasibility study on the search for $H\rightarrow ZZ^{*}\rightarrow 4 \mu$ at a muon collider is briefly exposed. Signal and Standard Model (SM) irreducible background processes are studied in two center-of-mass energy scenarios, 1.5 and 3 TeV, in order to present a first estimate of the sensitivity of the Higgs boson coupling to Z bosons achievable at this facility. The impact of the machine background (BIB), due to the decay of beam muons, is evaluated in the 1.5 TeV scenario.
\\\\At a multi-TeV muon collider, the Higgs boson would be produced mainly through Vector Boson Fusion (VBF)~\cite{ref:VBF}. However, it would be extremely complicated to measure the Higgs coupling to Z bosons ($g_{HZZ}$) in a process $\mu^{+} \mu^{-} \rightarrow H \mu^{+} \mu^{-}$, where the Higgs boson is produced through ZZ fusion. Indeed, the final state muons, which represent the experimental signature of such a process, would be emitted very forward, out of the acceptance region. Therefore, $H \rightarrow ZZ^{*}$ represents the favoured process to access the $g_{HZZ}$ coupling. 
\\The search for $H \rightarrow ZZ^{*} \rightarrow 4 \mu$ at a muon collider is investigated in two scenarios: $\sqrt{s}=$ 1.5 TeV and $\sqrt{s}=$ 3 TeV, which correspond, respectively, to the integrated luminosities of $L=$ 500 fb$^{-1}$ and $L=$ 1300 fb$^{-1}$. Signal and SM irreducible background MC samples, generated respectively with Pythia8~\cite{ref:pythia} and MadGraph~\cite{ref:madgraph}, are fully simulated and reconstructed with the software ILCSoft~\cite{ref:ILCSoft}. The simulated signal process is $\mu^{+} \mu^{-} \rightarrow H \nu_{\mu} \overline{\nu_{\mu}} \rightarrow Z Z^{*} \nu_{\mu} \overline{\nu_{\mu}} \rightarrow 4\mu \nu_{\mu} \overline{\nu_{\mu}}$, where the Higgs boson is produced through WW fusion, dominant mechanism at a multi-TeV muon collider. The SM background includes all the processes with four muons and two neutrinos in the final state: $\mu^{+} \ \mu^{-} \rightarrow 4\mu \ \nu_{\mu} \ \overline{\nu_{\mu}}$.
\\In the following, the most important aspects of the study are illustrated. First, the muon reconstruction performance is evaluated. A dedicated study on track reconstruction is carried out in order to estimate the impact of the BIB in the 1.5 TeV scenario. Then, a multivariate analysis (MVA) is performed in order to suppress the SM background in the signal region. The relative precision expected on the $g_{HZZ}$ coupling in the $4 \mu$ channel is finally computed.
\\At the Muon Collider, muon reconstruction is performed with Pandora Particle Flow Algorithms (PandoraPFA)~\cite{ref:PFA}, which combine hits collected and clustered in the calorimeter and tracks reconstructed essentially by means of the Conformal Tracking~\cite{ref:Conformal} and the Kalman filter~\cite{ref:Kalman} in the tracking system. The whole study on muon reconstruction performance, exposed in this section, is conducted by analyzing the four final state muons of the signal MC samples. The muon reconstruction efficiency and the transverse momentum ($p_{T}$) resolution are shown respectively in Fig.~\ref{fig:mureco} (left) and (right) as function of $p_{T}$. In order to provide more specific information about the reconstruction performance in different regions of the detector, three ranges of the polar angle $\theta$ are considered: 10$\degree$-20$\degree$, 20$\degree$-50$\degree$, 50$\degree$-90$\degree$. 
The reconstruction performance, which results in general very high, is found slightly degraded in the very forward region (10$\degree$-20$\degree$), since it is characterized by a transition between the detector layers of the tracking system.  


\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
        \includegraphics[width=\textwidth]{figures/phys_HZZ4mu_efficiency.eps}
        %\caption{Muon reconstruction efficiency as function of $p_{T}$ for three ranges of $\theta$.}
        %\label{fig:efficiency}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.45\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figures/phys_HZZ4mu_resolution.eps}
       %\caption{}
       %\label{fig:resolution}
   \end{subfigure}
   \caption{(left) Muon reconstruction efficiency and (right) $p_{T}$ resolution as function of $p_{T}$.}
   % for three ranges of $\theta$. }
   \label{fig:mureco}
\end{figure}

Previous results do not take into account the impact of the BIB on muon reconstruction, because of the high demanding computational resources needed for a full event reconstruction with the overlay. However, a shortcut is used in order to evaluate a preliminary effect of the BIB on track reconstruction, which is the most affected step of the reconstruction chain. The result of this study is shown in Fig.~\ref{fig:efficiency_BIB}, where the track reconstruction efficiencies evaluated with and without the BIB overlay are compared. %The impact of the BIB at 1.5 TeV is not huge and it is expected to result furtherly reduced at 3 TeV.
\begin{figure}[h]
\centering
  %\begin{minipage}[bl]{0.45\textwidth}
  \includegraphics[width=0.45\textwidth]{figures/phys_HZZ4mu_efficiencyBIB.eps}
  %\end{minipage}
  %\hfill
 % \begin{minipage}[br]{0.4\textwidth}
  \caption{Track reconstruction efficiency vs $p_{T}$, with and without the BIB overlay.} 
  \label{fig:efficiency_BIB}
  %\end{minipage}
\end{figure}

%\section{Analysis strategy and final results}
The analysis strategy developed for this study is inspired to the search for $H \rightarrow ZZ^{*} \rightarrow 4l$ performed by the CMS collaboration~\cite{ref:CMS} at LHC. Only events containing at least four good-quality final state muons with suitable electric charge are selected. In each of these events, two non overlapping Z candidates are built, sorted so that Z$_{1}$ corresponds to the muon pair with an invariant mass closest to the nominal value of the Z boson mass. ZZ candidates are then selected as explained in~\cite{ref:mio}. The mass distributions of the reconstructed Z$_{1}$ and Z$_{2}$ candidates are shown respectively in Fig.~\ref{fig:Zmass} (left) and (right) for signal and SM background.

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
        \includegraphics[width=\textwidth]{figures/phys_HZZ4mu_Z1mass.eps}
        %\caption{Muon reconstruction efficiency as function of $p_{T}$ for three ranges of $\theta$.}
        %\label{fig:efficiency}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.45\textwidth}
       \centering
       \includegraphics[width=\textwidth]{figures/phys_HZZ4mu_Z2mass.eps}
       %\caption{}
       %\label{fig:resolution}
   \end{subfigure}
   \caption{(left) $Z_{1}$  and (right) $Z_{2}$ mass distribution. }
   \label{fig:Zmass}
\end{figure}
The Higgs candidate is reconstructed as the combination of the two selected Z candidates.
A MVA analysis, based on angular distributions of the decay products of the Higgs boson, is carried out in order to discriminate the signal from its irreducible SM background. Fig.~\ref{fig:Higgs} shows the Higgs candidate mass distribution, obtained at the end of the whole selection, for signal and SM background.
\begin{figure}[h]
\centering
 %\begin{minipage}[bl]{0.45\textwidth}
  \includegraphics[width=0.45\textwidth]{figures/phys_HZZ4mu_Hmass.eps}
  %\end{minipage}
  %\hfill
  %\begin{minipage}[br]{0.4\textwidth}
   \caption{Higgs boson mass distribution normalized to cross section, luminosity and number of generated events.}
   \label{fig:Higgs}
 %\end{minipage}
\end{figure}
The relative precision expected on the $g_{HZZ}$ coupling is estimated, along with a projection of the effect of the BIB in the 1.5 TeV scenario. The $g_{HZZ}$ coupling is expected to be measured with a relative precision of 30$\%$  in the 1.5 TeV scenario, which worsens up to the 36$\%$ if the BIB is considered. Better precision could be achieved for a muon collider operating at $\sqrt{s}=$ 3 TeV. In this case, the $g_{HZZ}$ coupling would be measured in the 4$\mu$ channel with a 16$\%$ precision. An overall factor 2 improvement on the relative precision is expected if 4l (l=e,$\mu$) decay channel is considered. 

\subsection{$H\to \mu\mu$}
\hfill\textit{Alessandro Montella, Massimo Casarsa}\\

\noindent The measurement of the Higgs boson couplings to the second-generation fermions of the Standard Model is going to be one of the main objectives of the research programmes at the muon collider. A first feasibility study on the search for $H \rightarrow \mu^+ \mu^-$ is presented in this section, providing the first estimate of the muon collider reach on the measurement of $H \rightarrow \mu^+ \mu^-$ \cite{pos_hmumu}.

The study is carried out considering a 3-TeV muon collider and assuming an integrated luminosity of $1$ $\mathrm{ab}^{-1}$. Moreover, the study is performed without taking into account the effects of the BIB, which however are expected to have only a minimal impact on the muon reconstruction (see Section \ref{sec:muons}).

At a 3-TeV muon collider, the Higgs boson production is dominated by the $WW$-fusion, followed by the $ZZ$-fusion. Accordingly, the signal processes considered are the channels $\mu^+\mu^- \rightarrow H \nu_\mu \bar{\nu}_\mu$ ($H \rightarrow \mu^+\mu^-$) and $\mu^+\mu^- \rightarrow H \mu^+\mu^-$ ($H \rightarrow \mu^+\mu^-$). The background processes considered are the inclusive channels with the same final states as the signal (from which the signal channels have been excluded), and also a background via $t \bar{t}$ pair production in the s-channel: $\mu^+\mu^- \rightarrow \mu^+ \mu^- \nu_\mu \bar{\nu}_\mu$, $\mu^+\mu^- \rightarrow \mu^+\mu^-\mu^+\mu^-$ and $\mu^+\mu^- \rightarrow t \bar{t} \rightarrow W^+W^-b \bar{b}$ ($W^\pm \rightarrow \mu^\pm \nu_\mu [\bar{\nu}_\mu]$). The signal and background Monte Carlo samples are generated with MadGraph5 \cite{madgraph5} and Pythia8 \cite{pythia8}, and are processed with a full simulation of the muon collider detector and reconstructed using the Muon Collider Software \cite{mucolsoft}. The generation of the Monte Carlo samples is performed assuming a Standard Model Higgs boson with mass $m_H=125$ GeV and width $\Gamma_H = 4.07 \times 10^{U-3}$ GeV.

Before the event classification, an event preselection is performed in order to identify the potential Higgs boson event candidates as well as to suppress part of the low-energy background. The preselection requirements are provided in Figure \ref{tab1_hmumu}, and a stack of the distributions of the di-muon system invariant mass ($m_{\mu\mu}$) of the preselected events for the signal and background processes is shown in Figure \ref{fig1_hmumu}.
%

\begin{figure*}[!h]
  \begin{subtable}[b]{0.48\textwidth}
  \centering
     \begin{tabular}{cc} \hline
  \hline
Preselection requirements \\ \hline
Two opposite-charge muons \\
$10^\circ < \theta_{\mu} < 170^\circ$  \\
$105 < m_{\mu\mu} < 145 \; \mathrm{GeV}$ \\
$p_{T}(\mu^{\pm}) > 5 \; \mathrm{GeV} $ \\
$p_{T}(\mu^+\mu^-)>30 \; \mathrm{GeV}$ \\
$p_{T}(\mu^+)+p_{T}(\mu^-)>50 \; \mathrm{GeV}$  \\ \hline
$ $ \\
  \end{tabular}
  \caption{ }
  \label{tab1_hmumu}
  \end{subtable}
  %
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
  \includegraphics[width=1.0\linewidth]{figures/phys_Hmumu_InvMass.pdf} 
  \caption{ }
  \label{fig1_hmumu}
  \end{subfigure}
\caption{Summary of the preselection requirements (a), where $\theta$ is the polar angle and $p_T$ the transverse momentum; and stack of the distributions of $m_{\mu\mu}$ for the preselected signal and background events (b). }
\label{hmumu_mainfigure1}
\end{figure*}

The event classification is carried out using two multivariate classifiers based on a boosted decision tree (BDT). Each one of the two classifiers is trained independently to discriminate the signal against one of the two main backgrounds (\ie{} the backgrounds $\mu^+\mu^- \rightarrow \mu^+ \mu^- \nu_\mu \bar{\nu}_\mu$ and $\mu^+\mu^- \rightarrow \mu^+\mu^-\mu^+\mu^-$). Also, the training of the BDT classifiers is performed using a statistically independent sample from the one used for the statistical analysis, in orderd to avoid biases in the BDT outputs. 

The event selection is performed with the implementation of a double cut, which is applied to the classification scores obtained from the application of the two classifiers to the preselected events, in such a way as to select the events that are successfully discriminated against at least one of the two main backgrounds. The expected number of selected events is provided in Figure \ref{tab2_hmumu}, for each signal and background process, and a stack of the reconstructed $m_{\mu\mu}$ distributions of the selected events is shown in Figure \ref{fig2_hmumu}. The total signal selection efficiency is estimated to be $\epsilon_S=0.2667 \pm 0.007$.
%
\begin{figure*}[!h]
  \begin{subtable}[b]{0.48\textwidth}
  \centering\small\setlength\tabcolsep{.225em}
  \begin{tabular}{lc} \hline
  \hline
Process & \makecell{Expected events with\\  $105 < m_{\mu\mu} < 145$ GeV} \\ \hline
\makecell[l]{$\mu^+\mu^- \rightarrow H \nu_{\mu} \bar{\nu}_{\mu},$ \\$H \rightarrow \mu^+ \mu^-$} &  24.2 \\
\makecell[l]{$\mu^+\mu^- \rightarrow H \mu^+\mu^-,$\\ $H \rightarrow \mu^+\mu^-$} & 1.6 \\
$\mu^+\mu^- \rightarrow \mu^+\mu^-\nu\bar{\nu}_{\mu}$ & 636.5 \\
$\mu^+\mu^- \rightarrow \mu^+\mu^-\mu^+\mu^-$ & 476.4 \\
\makecell[tl]{$\mu^+\mu^- \rightarrow t \bar{t} \rightarrow W^+W^- b \bar{b},$\\ $W^{\pm} \rightarrow \mu^{\pm} \nu_{\mu}(\bar{\nu}_{\mu})$ } & 1.1 \\ \hline
  \end{tabular}
  \caption{ }
  \label{tab2_hmumu}
  \end{subtable}
  %
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
  \includegraphics[width=1.0\linewidth]{figures/phys_Hmumu_InvMass_BDTCut.pdf} 
  \caption{ }
  \label{fig2_hmumu}
  \end{subfigure}
\caption{Expected number of selected events in the invariant mass range from $105$ to $145$ GeV (a); and stack of the $m_{\mu\mu}$ distributions for the selected signal and background events (b). }
\label{hmumu_mainfigure2}
\end{figure*}

A convenient way to probe the Higgs boson coupling to the muon is by measuring the quantity $\sigma_H \times BR(H \rightarrow \mu\mu)$, which is determined from:
\begin{equation}
\sigma_H \times BR(H \rightarrow \mu\mu)= \frac{N_S}{L_{int} \cdot \epsilon_S},
\end{equation}
where $\sigma_H$ is the Higgs boson production cross section at a 3-TeV muon collider, $BR(H \rightarrow \mu\mu)$ the branching ratio of the $H \rightarrow \mu\mu$ decay channel, $N_S$ is the number of signal events in the range $105 < m_{\mu\mu}<145$ GeV, $L_{int}$ the assumed integrated luminosity and $\epsilon_S$ the total signal selection efficiency. The objective of this study is to estimate the sensitivity on the measurement of this quantity. The uncertainties on $L_{int}$ and $\epsilon_S$ are expected to be negligible compared to the uncertainty on $N_S$; accordingly, the uncertainty on $\sigma_H \times BR(H \rightarrow \mu\mu)$ is dominated by the statistical uncertainty on $N_S$, which is therefore taken as the estimate of the sensitivity of the measurement.

The number of signal events is extracted with an extended unbinned maximum likelihood fit to the $m_{\mu\mu}$ distribution with the function $f(m_{\mu\mu})=N_S \cdot f_S(m_{\mu\mu}) + N_B \cdot f_B(m_{\mu\mu})$, where $N_S$ and $N_B$ are taken as the free parameters of the fit ($N_B$ is the number of background events) and $f_S$ and $f_B$ are respectively the signal and background probability density functions, which are modeled independently with an unbinned maximum likelihood fit to the $m_{\mu\mu}$ distribution of the selected signal and background events, respectively.

The statistical uncertainty on $N_S$, $\sigma_{N_S}$, is estimated as the root mean square of the distribution of 10000 values of $N_S$ that are extracted from the $m_{\mu\mu}$ distribution of 10000 simulated pseudo-experiments. As a result, for a 3-TeV muon collider, the expected number of signal events in the $m_{\mu\mu}$ range from 105 to 145 GeV is expected to be $\langle N_S \rangle = 25.8 \pm 9.9$ for a dataset corresponding to an integrated luminosity of 1 $\mathrm{ab}^{-1}$. Accordingly, the relative uncertainty on $N_S$ is estimated as 
\begin{equation}
\frac{\sigma_{N_S}}{\langle N_S \rangle}=38\%
\end{equation}
and is taken as the estimate of the sensitivity on the measurement of $\sigma_H \times BR(H \rightarrow \mu\mu)$. Furthermore, this result can be substantially improved by implementing a more efficient strategy for the suppression of the background $\mu^+\mu^- \rightarrow \mu^+\mu^-\mu^+\mu^-$. For example, this background could be greatly reduced if the possibility to tag one of the two scattered muons from the initial state is enabled.

\subsection{$H\to bb$}
\hfill\textit{Laura Buonincontri}\\

\subsection{$H\to cc$ (no BIB)}
\hfill\textit{Paola Mastrapasqua, Rosamaria Venditti, Filippo Errico}\\
The Higgs Boson couplings to the second generations of fermions are of extreme interest due to sensitivity to a whole class of new physics models, but their measurement is extremely challenging, because of the small branching ratio. The coupling to charm quark, especially, is currently not accessible at LHC but could be probed at future lepton colliders.\\
A first feasibility study on the search for  $H \rightarrow c\bar{c}$ at Muon Collider has been performed. The $\mu^{+} \mu^{-} \rightarrow H \nu\bar{\nu} \rightarrow c\bar{c} \nu\bar{\nu} $ signal process has been fully simulated and reconstructed at $\sqrt{s}=1.5 $ TeV, along with the main physics backgrounds, while for the time being the BIB is not included.
The resonant background consists of Higgs Boson decays to a pair of bottom quarks ($H \rightarrow b \bar{b}$) and to a pair of gluons ($H\rightarrow gg$), whose branching ratios are respectively 20 and 3 times higher than the signal one. The non-resonant background is represented by processes with two jets and two leptons of any kind in the final states.
Signal and background processes are generated using Pythia8 \cite{ref:Pythia} and MadGraph5 \cite{ref:MG}. The Muon Collider detector response simulation and reconstruction are performed with ILCSoft \cite{ref:ILCSoft}. \\

MAYBE THIS COULD GO IN THE "HEAVY-FLAVOR JET" SECTION \\

In order to discriminate c jets from b jets and light-flavour jets, a dedicate tagger has been implemented, exploiting the properties of heavy-flavour hadrons resulting from radiation and hadronization of charm quarks. The sizeable lifetime of these hadrons together with their relativistic boost give rise to displaced tracks (large signed impact parameter, SIP) and secondary vertices (SVs) millimetres or more away from the primary one. Moreover the semi-leptonic decays of heavy hadrons lead to the presence of non-isolated low-energy electrons and muons, collectively called soft leptons. For these reasons, the tagger relies on three types of variables: secondary vertex related variables (examples in Figure \ref{pic:vertex_cat}), track related variables (example in Figure \ref{pic:trk} left) and soft lepton related variables (example in Figure \ref{pic:trk} right). 
\\Two binary Boosted Decision Tree classifiers have been trained: one for discriminating c jets from b jets (\textit{CvsB}) and the other for discriminating c jets against light-flavour jets (\textit{CvsL}). The performances of the two separate classifiers compared to the CMS and CLIC ones are reported in Ref. \cite{Hcc_proceeding}. Since the two discriminators are applied together in the analysis, it is helpful to evaluate their combined effect on signal and backgrounds and calculate the total tagging efficiency and mis-tagging probability as shown in Figure \ref{pic:minv} left. The working point chosen for the analysis lies on the 40$\%$ charm efficiency curve (magenta line, labeled with "3") in correspondence of 5$\%$ light-flavour and 13$\%$ bottom contamination.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
        \includegraphics[width=0.99\textwidth]{figures/phys_c_tagger_vtx_cat.eps}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.45\textwidth}
       \centering
       \includegraphics[width=0.99\textwidth]{figures/phys_c_tagger_SV_fd.eps}
   \end{subfigure}
   \caption{(Left) Jet fraction per vertex category. The "NoVertex" category contains jets with no SV, while the "RecoVertex" category contains jets with at least a SV in it. (Right) 3D flight distance divided by its uncertainty (significance) for the first SV. SVs are ordered by increasing uncertainty on their 3D flight distance.}
   \label{pic:vertex_cat}
\end{figure}


\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
        \includegraphics[width=0.99\textwidth]{figures/phys_c_tagger_track_SIP.eps}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.45\textwidth}
       \centering
       \includegraphics[width=0.99\textwidth]{figures/phys_c_tagger_lep_pt.eps}
   \end{subfigure}
   \caption{(Left) 2D SIP divided by its uncertainty (significance) for the second track. Tracks are ordered by decreasing 2D SIP significance. (Right) Transverse momentum of the first lepton divided by jet transverse momentum. Leptons are ordered as tracks.}
   \label{pic:trk}
\end{figure}

The highest-$p_{T}$-jets surviving the flavour tagging are used to build the Higgs candidates. Several topological selection are applied in order to suppress the prompt jet background: the separation between jets in the $\eta-\phi$ plane is required to be smaller than 3, the Higgs candidate is required to have energy greater than 130 GeV, $p_{T}$ greater than 30 GeV, and invariant mass in the range $\left[110,130\right]$ GeV. Figure \ref{pic:minv} right shows the mass distribution for the signal and backgrounds surviving the event selection, i.e. the resonant component and the prompt c jet production.
\\The final number of expected signal events (S) and background events (B) are used for computing approximatively the relative uncertainty on the $H \rightarrow c \bar{c}$ production cross section and on the Higgs-to-c-quark coupling, following Ref. \cite{ref:MuColl2}.
Table \ref{tab:results} summarizes the results and shows the projection at $\sqrt{s} = 3$ TeV, $\mathcal{L} = 1300$ fb$^{-1}$, obtained assuming the same fraction of surviving events per each sample and scaling the results to cross section and luminosity at the increased center of mass energy. These estimates are very preliminary but already show the potential of the Muon Collider, if an efficient machine background mitigation strategy is adopted. \\

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    	\centering
        \includegraphics[width=0.99\textwidth]{figures/phys_c_tagger_eff_contour.eps}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.45\textwidth}
       \centering
       \includegraphics[width=0.99\textwidth]{figures/phys_H_cc_inv_mass.eps}
   \end{subfigure}
   \caption{(Left) Misidentification probability for light-flavour jets versus misidentification probability for b jets for several constant c jet efficiencies. (Right) Invariant mass of the di-jet system for the processes surviving the selections. The selected mass range is indicated by the vertical dashed lines. Histograms are scaled to cross section and luminosity.}
   \label{pic:minv}
\end{figure}


\begin{table}[h!]
	\centering
    \begin{tabular}{ccccccc} 
    \hline
    \rule{0mm}{3mm}
	$\boldsymbol{\sqrt{s}} \; \left[ TeV \right]$ & $\boldsymbol{\mathcal{L}} \; \left[ fb^{-1} \right]$ & \textbf{   S   } & \textbf{   B   } & $\boldsymbol{S/\sqrt{S+B}}$ &   $\boldsymbol{\Delta\sigma/\sigma}$   &   $\boldsymbol{\Delta g_{Hcc}/g_{Hcc}}$ \\
	\hline
	1.5 & 500 & 378 & 1205 & 9.5 & 10.5 $\%$ & 5.5 $\%$ \\
	3.0 & 1300& 1565 & 4337 & 20.4 & 4.9 $\%$ & 2.6 $\%$ \\
	\hline
	\end{tabular}
	\caption{Signal and background yields, signal significance, relative uncertainty on $H \rightarrow c\bar{c}$ production cross section and relative uncertainty on the Hcc coupling at 1.5 and 3 TeV, without BIB overlay. }
	\label{tab:results}
\end{table}





\subsection{$HH\to 4b$}
\hfill\textit{Laura Buonincontri, Lorenzo Sestini}\\

\subsection{Dark SUSY in the Muon Spectrometer}
\hfill\textit{Chiara Aim\'e, Cristina Riccardi}\\

\subsection{Disappearing track (already published)}
\hfill\textit{Federico Meloni}\\

\subsection{Heavy (meta-)stable charged particles}
\hfill\textit{Simone Pagan Griso}\\
